ASSURED: Architecture for Secure Software Update of Realistic Embedded Devices

Secure firmware update is an important stage in the IoT device life-cycle. Prior techniques, designed for other computational settings, are not readily suitable for IoT devices, since they do not consider idiosyncrasies of a realistic large-scale IoT deployment. This motivates our design of ASSURED, a secure and scalable update framework for IoT. ASSURED includes all stakeholders in a typical IoT update ecosystem, while providing end-to-end security between manufacturers and devices. To demonstrate its feasibility and practicality, ASSURED is instantiated and experimentally evaluated on two commodity hardware platforms. Results show that ASSURED is considerably faster than current update mechanisms in realistic settings.

==> sections/related.tex <==
\section{Related Work}
\label{sec:related-work}
Due to space constraints, we limit the discussion in this section to prior work in the area of secure 
updates for low-end devices. A much more thorough overview of related work in remote attestation 
can be found in~\cite{abera2016things}.




Several prior secure update techniques use pre-existing remote attestation designs. For example, 
\emph{SCUBA}~\cite{seshadri2006scuba} can be used to repair a compromised sensor 
through firmware updates.
SCUBA utilizes an authentication mechanism and software-based attestation to identify 
memory regions infected by malware and transmits the repair update to replace these regions.
However, the attestation technique based on self-checksumming code heavily relies on
consistent timing characteristics of the measurement process the use of an optimal checksum function. 
These assumptions  do not make SCUBA a suitable approach for IoT settings~\cite{castelluccia2009difficulty}.

Perito and Tsudik~\cite{perito2010secure} present a simple secure firmware update technique using so-called
Proofs of Secure Erasure (PoSE-s). The idea is for prover (\dev) to perform secure erasure before retrieving and 
installing a new update, from clean slate.  Secure erasure is achieved by filling all of prover's memory with 
(uncompressable) randomness chosen by verifier. Prover then returns a snapshot of the new memory contents
to verifier as a proof of secure erasure. This proof guarantees that prover is now in a benign state and ready to perform 
an update. However, all PoSE-based update techniques only work in a one-hop prover/verifier setting. Furthermore,
they do not support {\em robust updates}, i.e. ability to retain previous version(s), in case a roll-back is
required, e.g., if the current update cannot be successfully completed. Whereas, in \acro, \dev 
can isolate untrusted software, thus secure erasure is not needed and update robustness can be achieved.




==> sections/response.tex <==
\newpage
\clearpage
\onecolumn
\section*{Response to Reviewers}
We thank all reviewers for their valuable and insightful comments. Please find our responses below.



\subsection*{Reviewer \#1}

Reviewer \#1's comments are addressed below, under ``Other Changes".


\subsection*{Reviewer \#2}

\Que{Add some performance comparison with UPTANE platform.}

\Ans{To the best of our knowledge, there is no official (public) C implementation of Uptane. The reference implementation
available from:  \url{https://github.com/uptane/uptane} is written in Python. Thus, it is not practically feasible for us to port it to a
resource-constrained embedded platform, in order to facilitate comparative performance analysis. After we submitted this paper, 
an unofficial C implementation has appeared: \url{https://github.com/samlauzon/libuptane}. However, it still is {\em work-in-progress} 
and is rather incomplete.}

\subsection*{Reviewer \#3}

\Que{Clarify how the architecture addresses the threat model. Have more discussion about how the stated 
objectives are met inline in the text, specifically, in Sec. 4 on the design.}

\Ans{We clarified how we meet our stated objectives in Section~\ref{sec:design}. In particular, we describe 
how specific design decision address the stated objectives of Sections~\ref{sec:soe} and~\ref{sec:auth-mechanism}.}

\Que{Include experimental results on the performance of the DC. What is the cost of the computation being pushed 
from the device to the DC?}

\Ans{We clarified the computational cost for \dc in Figure~\ref{fig:runtime-lowfreq} and included \acro run-time on
\dc in Section~\ref{sec:eval}.}

\subsection*{Reviewer \#4}

\Que{Dive into the evaluation more.  What \% of improvements are from optimizations that could equally 
be applied to TUF?}

\Ans{We clarified this in Section~\ref{sec:eval}. If we were to modify TUF to support a similar encoding scheme, 
TUF performance would be improved by around 6\%. We now mention this in Section~\ref{sec:eval}.} 

\Que{Better justify why the performance benefits matter, especially when taken with the increased exposure 
the system gets from integrating the DC into the system.}

\Ans{Integration of \dc into the system does \emph{not} weaken security or increase exposure; the device (\dev) implements the necessary mechanisms to meet OEM requirements 
of end-to-end security (\fbox{O1}), update authorization (\fbox{O2}) and attestation (\fbox{O3}). In other words, \acro provides security similar to that of TUF. It also satisfies additional OEM requirements on 
update distribution.
\acro can be seamlessly combined with TUF infrastructure on \dc, to benefit from security guarantees 
provided by TUF. For instance, \acro relies on TUF at \dc for update freshness by verifying that the timestamp TUF's metadata is fresh. We clarify this in the beginning of  Section~\ref{sec:design}.

Improved performance  -- together with fewer keys and less metadata needed to be stored on \dev (\fbox{O5}) -- 
yield several benefits that improve deployability of \acro, as compared to TUF and Uptane. As we argue in 
Section~\ref{sec:our-goals}, the biggest hurdle for TUF deployability in resource-constrained settings is the need to place complex logic and 
PKI on \dev, a requirement that makes Uptane unsuitable for deployment in automotive settings, 
or any system that includes a broad range of devices, not all of which can download and verify all TUF metadata. 

Uptane overcomes this issue through the realization that different computing units can conduct metadata verification 
in different ways, which allows Uptane to relax verification requirements for resource-constrained devices. However,
Uptane, is inflexible from deployment perspective, since it was designed primarily to facilitate automotive updates.
Whereas, \acro is designed to provide more flexibility in terms of types, scale and operational policies. 
We adjusted the wording in Section~\ref{sec:our-goals} in order to more clearly delineate the differences between \acro and 
previous work.}

\Que{Compare to more systems, as in the embedded community, I don't know of consensus for TUF being "the system" to beat. 
If it is, then it should be justified as such.}

\Ans{TUF (and its variants) are being deployed in real-world IoT scenarios, e.g., in the automotive industry~\cite{uptane-news}. 
Furthermore, TUF is currently one of the few established standards for IoT settings, while other standardization efforts are ongoing. TUF is also the secure software update framework that is freely available.
We clarified this in Section~\ref{sec:eval}.}

\Que{Citations or real systems that justify why the stakeholders and objectives aren't created specifically to motivate this problem? 
Why are they a "real problem"?}

\urldef\urlmoranseca\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-3.2}
\urldef\urlmoransecb\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-3.3}
\urldef\urlmoransecc\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-3.9}
\urldef\urlmoransecd\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-3.6}
\urldef\urlmoransece\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-3.7}
\urldef\urlmoransecf\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00#section-9}

We use the model of "stakeholders" for IoT firmware updates introduced in the {\em "Software Updates for Internet of Things"} (SUIT) working 
group of the IETF\footnote{\url{https://datatracker.ietf.org/wg/suit/about/}}. The original model and objectives are documented in the 
Internet-Draft by Moran et al.\footnote{\url{https://tools.ietf.org/html/draft-ietf-suit-architecture-00}} describing specifications and 
requirements of firmware update mechanisms for embedded devices. Specifically, \acro's \oem and \sd corresponds to "Author" and 
"Untrusted Storage" entities, respectively. The needs for \dc to enforce update policies on the device are discussed by Moran et al. in 
Section 3.9\footnote{\urlmoransecc}. 
Note that \dc  acts as an agent for a device operator, network operator or device owner. These requirements have been verified in 
discussion with various industry representatives, although the exact entities involved in update policy naturally varies across concrete 
IoT device deployment use-cases. In case of consumer devices, such as wearables, \dc is likely to represent the device owner, and 
could be realized as a component in a personal computing device, e.g., a smartphone. We clarified the relationship between our 
stakeholder model and requirements identified by industry standardization efforts in Section~\ref{sec:stakeholders}.

Our stated objectives are consistent with the requirements identified by Moran et. al. 
\begin{compactitem}
\item \fbox{O1} combines requirement  "Friendly to broadcast delivery" (Section 3.2\footnote{\urlmoranseca}) and 
"Use of state-of-the-art security mechanism" (Section 3.3\footnote{\urlmoransecb}).
\item \fbox{O2} is based on requirement "Robust permissions" (Section 3.9\footnote{\urlmoransecc}).
\item \fbox{O5} is based on requirements "Operate with a small bootloader" (Section 3.6\footnote{\urlmoransecd}), 
"Small parsers" (Section 3.7\footnote{\urlmoransece}), and additional deployment considerations out of scope of
Moran et al., but discussed in our Section 9\footnote{\urlmoransecf}. 
\item \fbox{O3} is based on the notion that, for IoT deployments targeted by \acro, it is is essential for \dc (acting on behalf 
of device operator or owner) to reliably learn the outcome of the update process, in order to maintain operational integrity and auditability.
In particular, \fbox{O3} allows \dc to detect conditions that cause the update process to fail, 
e.g., MitM attacker between Device and Controller prevents an update from reaching \dev.
\item \fbox{O4} follows from \fbox{O3}. 
\end{compactitem}
We clarified the relationship between our stated objects and the stakeholder model in Sections~\ref{sec:our-goals} and~\ref{sec:design}.

\subsection*{Other Changes}

\begin{itemize}
  \item In response to a comment  by Reviewer \#1, added a new subsection (Section~\ref{sec:boot-integrity} )
  on "Boot Integrity" that overviews established secure and authenticated boot mechanisms, their applicability to embedded devices, 
  especially to resource-constrained MCU platforms, and discusses the  relationship between authenticated boot and remote attestation.
    
  \item In response to comments about excessive use of abbreviations by Reviewers \#1 and \#4, 
  replaced references $Dev$, $DC$ and $SD$ throughout the manuscript with \dev, \dc, and \sd, respectively, 
  and adjusted when these terms are introduced.
  
  \item In response to comment by Reviewer \#1, added discussion in Section~\ref{sec:soe} on limitations of \acro, and elaborated 
  on how it addresses specific threats, e.g., how \dc can detect if \dev is compromised by the attacker and as a result, is not performing requested updates.
   
  \item In response to comment by Reviewer \#3, added Figure~\ref{fig:tuf-uptane} illustrating (at a high-level) operation of TUF 
  and Uptane to support the discussion on related techniques. 
  
  \item Based on comments by Reviewers \#2, \#3, and \#4, fixed the issues with Figure~\ref{fig:update} (previously Figure 1), i.e., 
  recognizability of glyphs, typo in "Remote Connectivity" and visibility of "Authenticated channel" annotation when viewed in black-and-white.
    
  \item In response to request for clarification by Reviewer \#4, clarified the meaning of "constraints" with new examples in Section~\ref{sec:stakeholders}.
    
  \item Per Reviewer \#4's request, fixed footnote numbering on pages 6 and 7.
  
  \item Finally, fixed various minor typos throughout the manuscript.
  
\end{itemize}



